Multi-Flow Attacks Against Network Flow Watermarks: Analysis and Countermeasures

In this paper, we analyze several recent schemes for watermarking network flows that are based on splitting the flow into timing intervals. We show that this approach creates time-dependent correlations that enable an attack that combines multiple watermarked flows. Such an attack can easily be mounted in nearly all applications of network flow watermarking, both in anonymous communication and stepping stone detection. The attack can be used to detect the presence of a watermark, recover the secret parameters, and remove the watermark from a flow. The attack can be effective even if different flows are marked with different values of a watermark. We analyze the efficacy of our attack using a probabilistic model and a Markov-Modulated Poisson Process (MMPP) model of interactive traffic. We also implement our attack and test it using both synthetic and real-world traces, showing that our attack is effective with as few as 10 watermarked flows. Finally, we propose possible countermeasures to defeat the multi-flow attack.

==> cm-new.tex <==
\section{Countermeasures}

We now proceed to consider some countermeasures to the multi-flow attack.  Overall, the multi-flow attack
relies on being able to find flows that are marked in similar ways.  We consider countermeasures that vary some of the watermarking parameters in order to make our attack more difficult.  In principle, this is a well-founded approach: by varying parameters, the attacker's task can be made much more difficult, since an exponential search may be necessary to find a configuration of flows that exhibit the same choice of parameters.  However, in some cases, the actual extend of the search is still small enough to remain practical; we analyze the relative impact of the choice of varying parameters on the attack.

We analyze two types of attack: watermark presence detection and watermark parameter recovery.  Note that our attack on unmodified interval-based schemes easily accomplishes both, by identifying matching clear intervals in the watermarked flows.  However, in general, the latter problem is significantly more difficult.  Detecting the presence of watermark can be seen to be equivalent to decoding \emph{identification codes}, blah blah blah...


\subsection{Varied Offset}

The simplest parameter to vary in flow watermarking is the initial offset, $o$.  In fact, several of the schemes we analyzed suggest that the offset be chosen randomly in some interval $[0,o_{max}]$ (typically, $o_{max} = T$).  This is because the watermarking schemes can be re-synchronized: the detector iteratively performs the watermark recognition algorithm uses offsets in the range $[0,o_{max}]$, stepping through offsets by the interval $\delta$.  $\delta$ needs to be chosen small enough such that a mismatch of $\delta$ between the offsets used in encoding and decoding does not prevent the watermark from being detected, and large enough such that the number of decoding operations, $\lceil o_{max} / \delta \rceil$, does not introduce 
undue computational overhead.  If the watermark is detected at any of the offsets, the flow is considered to be watermarked.

The use of multiple offsets increases both the false positives and false negative rates; both of these depend on $o_{max}$ and $\delta$ in non-trivial ways.  However, it is possible to bound the increase in false positives by a factor of $\lceil o_{max} / \delta$.  In practice, this does not have a very large impact on the watermark performance; XXX empirically analyzed offset synchronization in their scheme and found that XXX.

To adapt the multi-flow attack to the multi-offset scheme, we can perform a similar search for the correct offset.  
To adjust for a possible mismatch of length $\delta$, we look for intervals of length $T - \delta$.  This will increase the chance of false positives we need to consider, since smaller intervals have a higher chance of being clear in a non-watermarked flows.  In addition, for each flow, we will need to consider $\lceil o_{max} / \delta \rceil$ positions.  Therefore, the overall possibility of a false positive, given $k$ flows that have matching intervals of length $T-\delta$, is bounded by:

\[ \lceil o_max / \delta \rceil^k \cdot P_{f_{m}}(0; T-\delta) \]

For example, assuming $T = 0.9$ (as in~\cite{pyun+:oakland07}) and $o_{max} = T$, we can set $\delta = T/2$.  In this case, we can solve for $k$:

\[ \lceil o_max / \delta \rceil^k \cdot P_{f_{m}}(0; T-\delta)^k < \epsilon \]
\[ 2^k P_{f_{m}}(0;0.45)^k < \epsilon \]
\[ k > \log_{2 \cdot 0.276} \epsilon \]

Thus, to achieve an error rate of $< 10^{-5}$, we need to use $k = 20$ flows.  For larger $o_{max}$ and smaller $T$, it may in fact be impossible to avoid false positives; for example, using $T = 0.35$, $P_{f_m}(0;T/2) = 0.525$.  Thus, even with $\delta = T/2$ and $o_{max} = T$, there is no solution, because $2 \cdot P_{f_m}(0;0.175) > 1$.  This suggests that picking $o_{max} > T / (2\cdot P_{f_m}(0;T/2))$ may be an effective offset-based countermeasure 

Using multiple offsets also increase the computational burden on the attacker; in the former case, the attacker must consider $2^{20}$ different combinations of offsets.  In practice, this search space can be reduced by a branch-and-bound algorithm that iteratively builds up larger collections of flows and increases the 

Thus, to achieve a false error rate of $10^{-5}$, we need to set $k = 
In our case, we set $\delta = T/2$, and rather than looking for clear intervals of length $T$, we look for intervals of length $T/2$.  This will increase the number of flows we will need to consider in order to detect a multi-flow attack.  For example, as described in \S XXX, $P_{f_{m}}(0; 0.35) \approx 0.33$, so $P_{f_{m}}(0; 0.35)^{10} = 1.6 \times 10^{-5}$; i.e., the probability of finding a clear interval of length 350ms in 10 non-watermarked flows is $1.6 \times 10^{-5}$.  The probability of a clear interval of length 175ms, on the other hand, is $P_{f_m}}(0;0.175) \approx 0.52$, thus 10 flows might have a matching clear interval of length 175ms with probability $\approx 1.6 \times 10^{-3}$.  

In addition, because multiple combinations of flows are attepmted, the probability of a false positive increases.  Given $k$ flows, we must try all $o_{max} / \delta$ choices of offsets for each flow.  This creates a search space of $\lceil o_{max} / \delta \rceil^k$.  Assuming that $o_{max} = T$, it is easy to see that, with 



==> figures/10flows-ning.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{figures/10flows-ning}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,10800)(0,0)%
\put(825,1100){\makebox(0,0){\strut{} 0}}%
\put(4095,1100){\makebox(0,0){\strut{} 2}}%
\put(7365,1100){\makebox(0,0){\strut{} 4}}%
\put(10635,1100){\makebox(0,0){\strut{} 6}}%
\put(13905,1100){\makebox(0,0){\strut{} 8}}%
\put(17175,1100){\makebox(0,0){\strut{} 10}}%
\put(9000,275){\makebox(0,0){\strut{}Time (s)}}%
\put(14950,9675){\makebox(0,0)[r]{\strut{}10 flows}}%
\put(14950,9125){\makebox(0,0)[r]{\strut{}10 watermarked flows}}%
\end{picture}%
\endgroup
\endinput


==> figures/10flows.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{figures/10flows}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,10800)(0,0)%
\put(825,1100){\makebox(0,0){\strut{} 0}}%
\put(4095,1100){\makebox(0,0){\strut{} 1}}%
\put(7365,1100){\makebox(0,0){\strut{} 2}}%
\put(10635,1100){\makebox(0,0){\strut{} 3}}%
\put(13905,1100){\makebox(0,0){\strut{} 4}}%
\put(17175,1100){\makebox(0,0){\strut{} 5}}%
\put(9000,275){\makebox(0,0){\strut{}Time (s)}}%
\put(14950,9675){\makebox(0,0)[r]{\strut{}10 flows}}%
\put(14950,9125){\makebox(0,0)[r]{\strut{}10 watermarked flows}}%
\end{picture}%
\endgroup
\endinput


==> figures/bulk.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{bulk}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,10800)(0,0)%
\put(825,1100){\makebox(0,0){\strut{} 0}}%
\put(4095,1100){\makebox(0,0){\strut{} 1}}%
\put(7365,1100){\makebox(0,0){\strut{} 2}}%
\put(10635,1100){\makebox(0,0){\strut{} 3}}%
\put(13905,1100){\makebox(0,0){\strut{} 4}}%
\put(17175,1100){\makebox(0,0){\strut{} 5}}%
\put(9000,275){\makebox(0,0){\strut{}Time (s)}}%
\put(14950,9675){\makebox(0,0)[r]{\strut{}10 flows}}%
\put(14950,9125){\makebox(0,0)[r]{\strut{}10 watermarked flows}}%
\put(14950,8575){\makebox(0,0)[r]{\strut{}1 watermarked flow}}%
\end{picture}%
\endgroup
\endinput


==> figures/bulk2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,665){\makebox(0,0)[r]{\strut{} 0}}%
      \put(990,1121){\makebox(0,0)[r]{\strut{} 100}}%
      \put(990,1578){\makebox(0,0)[r]{\strut{} 200}}%
      \put(990,2035){\makebox(0,0)[r]{\strut{} 300}}%
      \put(990,2492){\makebox(0,0)[r]{\strut{} 400}}%
      \put(990,2949){\makebox(0,0)[r]{\strut{} 500}}%
      \put(990,3406){\makebox(0,0)[r]{\strut{} 600}}%
      \put(990,3862){\makebox(0,0)[r]{\strut{} 700}}%
      \put(990,4319){\makebox(0,0)[r]{\strut{} 800}}%
      \put(990,4776){\makebox(0,0)[r]{\strut{} 900}}%
      \put(1122,440){\makebox(0,0){\strut{} 0}}%
      \put(2263,440){\makebox(0,0){\strut{} 1}}%
      \put(3404,440){\makebox(0,0){\strut{} 2}}%
      \put(4544,440){\makebox(0,0){\strut{} 3}}%
      \put(5685,440){\makebox(0,0){\strut{} 4}}%
      \put(6826,440){\makebox(0,0){\strut{} 5}}%
      \put(220,2718){\rotatebox{90}{\makebox(0,0){\strut{}Rate (pkt/s)}}}%
      \put(3974,110){\makebox(0,0){\strut{}Time (s)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4603){\makebox(0,0)[r]{\strut{}10 flows}}%
      \csname LTb\endcsname%
      \put(5839,4383){\makebox(0,0)[r]{\strut{}10 watermarked flows}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/bulk2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/bulk3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,665){\makebox(0,0)[r]{\strut{} 0}}%
      \put(990,1121){\makebox(0,0)[r]{\strut{} 100}}%
      \put(990,1578){\makebox(0,0)[r]{\strut{} 200}}%
      \put(990,2035){\makebox(0,0)[r]{\strut{} 300}}%
      \put(990,2492){\makebox(0,0)[r]{\strut{} 400}}%
      \put(990,2949){\makebox(0,0)[r]{\strut{} 500}}%
      \put(990,3406){\makebox(0,0)[r]{\strut{} 600}}%
      \put(990,3862){\makebox(0,0)[r]{\strut{} 700}}%
      \put(990,4319){\makebox(0,0)[r]{\strut{} 800}}%
      \put(990,4776){\makebox(0,0)[r]{\strut{} 900}}%
      \put(1122,440){\makebox(0,0){\strut{} 0}}%
      \put(2263,440){\makebox(0,0){\strut{} 1}}%
      \put(3404,440){\makebox(0,0){\strut{} 2}}%
      \put(4544,440){\makebox(0,0){\strut{} 3}}%
      \put(5685,440){\makebox(0,0){\strut{} 4}}%
      \put(6826,440){\makebox(0,0){\strut{} 5}}%
      \put(220,2718){\rotatebox{90}{\makebox(0,0){\strut{}Rate (pkt/s)}}}%
      \put(3974,110){\makebox(0,0){\strut{}Time (s)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4603){\makebox(0,0)[r]{\strut{}1 watermarked flow}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/bulk3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/diffkey.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{figures/diffkey}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,10800)(0,0)%
\put(825,1100){\makebox(0,0){\strut{} 0}}%
\put(4095,1100){\makebox(0,0){\strut{} 1}}%
\put(7365,1100){\makebox(0,0){\strut{} 2}}%
\put(10635,1100){\makebox(0,0){\strut{} 3}}%
\put(13905,1100){\makebox(0,0){\strut{} 4}}%
\put(17175,1100){\makebox(0,0){\strut{} 5}}%
\put(9000,275){\makebox(0,0){\strut{}Time (s)}}%
\put(14950,9675){\makebox(0,0)[r]{\strut{}0,1,2,3,4,5,6,7,8,10,11}}%
\put(14950,9125){\makebox(0,0)[r]{\strut{}0,1,2,3,5,8,10,12,16,17}}%
\put(14950,8575){\makebox(0,0)[r]{\strut{}0,1,2,4,6,7,10,12,13,14}}%
\put(14950,8025){\makebox(0,0)[r]{\strut{}0,1,5,6,8,9,10,12,14,15}}%
\end{picture}%
\endgroup
\endinput


==> figures/diffkey2.tex <==
%GNUPLOT: LaTeX picture with Postscript
\begin{picture}(0,0)%
\includegraphics{figures/diffkey2}%
\end{picture}%
\begingroup
\setlength{\unitlength}{0.0200bp}%
\begin{picture}(18000,10800)(0,0)%
\put(825,1100){\makebox(0,0){\strut{} 700}}%
\put(4095,1100){\makebox(0,0){\strut{} 701}}%
\put(7365,1100){\makebox(0,0){\strut{} 702}}%
\put(10635,1100){\makebox(0,0){\strut{} 703}}%
\put(13905,1100){\makebox(0,0){\strut{} 704}}%
\put(17175,1100){\makebox(0,0){\strut{} 705}}%
\put(9000,275){\makebox(0,0){\strut{}Time (s)}}%
\put(14950,9675){\makebox(0,0)[r]{\strut{}0,1,2,3,4,5,6,7,8,10,11}}%
\put(14950,9125){\makebox(0,0)[r]{\strut{}0,1,2,3,5,8,10,12,16,17}}%
\put(14950,8575){\makebox(0,0)[r]{\strut{}0,1,2,4,6,7,10,12,13,14}}%
\put(14950,8025){\makebox(0,0)[r]{\strut{}0,1,5,6,8,9,10,12,14,15}}%
\end{picture}%
\endgroup
\endinput


==> figures/dsss.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,660){\makebox(0,0)[r]{\strut{} 0}}%
      \put(990,1483){\makebox(0,0)[r]{\strut{} 50}}%
      \put(990,2306){\makebox(0,0)[r]{\strut{} 100}}%
      \put(990,3130){\makebox(0,0)[r]{\strut{} 150}}%
      \put(990,3953){\makebox(0,0)[r]{\strut{} 200}}%
      \put(990,4776){\makebox(0,0)[r]{\strut{} 250}}%
      \put(1122,440){\makebox(0,0){\strut{} 0}}%
      \put(2263,440){\makebox(0,0){\strut{} 2}}%
      \put(3404,440){\makebox(0,0){\strut{} 4}}%
      \put(4544,440){\makebox(0,0){\strut{} 6}}%
      \put(5685,440){\makebox(0,0){\strut{} 8}}%
      \put(6826,440){\makebox(0,0){\strut{} 10}}%
      \put(220,2718){\rotatebox{90}{\makebox(0,0){\strut{}Rate (pkt/s)}}}%
      \put(3974,110){\makebox(0,0){\strut{}Time (s)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/dsss}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> literature.tex <==

\section{More literature}






Jia et al. in \cite{conf/infocom/JiaTLFXY09} use the known concepts in the filed of spread spectrum communications to design a new attack on the DSSS flow watermarking scheme of \cite{yu:oakland07} which is based on spread spectrum watermarking. Their attack is able to detect a using a single network flow, but it only works for the watermarking scheme of \cite{yu:oakland07}.




Pdhye et~al.\  design SNEAK a method that attackers can use to evade the detection of their use of stepping stones\cite{padhye:elsv10}.  Using enough buffering and addition of chaff packets at the stepping stones, SNEAK manipulates the outbound flow toward a constant rate flow, trying to destroy all the timing correlations between the flow entered the stepping stone, and the one leaving it. This method, however, requires full access on the stepping stone hosts by the attackers, and also may result in large delays, due to the buffering, for certain types of the traffic. In addition, observation of constant rate flows can be used as a sign of abnormality by network defenders. 


Coskun et~al.\ in \cite{conf/acsac/CoskunM09} propose a new approach for detection of stepping stones, based on succinct packet-timing sketches of network flows. A border router evaluates the sketches of the observed flows online, trying to pair correlated network flows. The scheme is more scalable, compared to similar passive detection schemes, as the detection of correlated flows is done in sub-quadratic time. Also, the succinct flow sketches enable the
detection scheme to compare a given pair of flows in constant time. The detection rates, however, are not comparable with those of watermark-based detections, while chaff and delays make the detection performance even worse. 

Wang et~al. in \cite{conf/ccs/WangMS08} propose a dependent link padding scheme in order to protect anonymity systems from traffic analysis. The scheme results in a bounded delay and required different rates of covering traffic for different types of flows. 


Pries et al. design \textit{replay attack}, a new approach for compromising the anonymity of TOR \cite{conf/icc/PriesYFZ08}. The attack works by a malicious entry node duplicating and sending the TOR traffic, which could result in some errors at the TOR exit node that tries to decrypt the cells. If this exit node is also controlled by an accomplice, the attackers are able to link the sender and receiver of that specific flow. The scheme has limited capabilities, as the attacker needs to  control both entry and exit nodes. The replay attack can also be used as a means for DoS attacks. 

Park et al. in \cite{Park07} and \cite{park:ICICS07}  propose adaptive flow watermarking approaches, in order to decrease the redundancy required to achieve some detection accuracy. Two methods are proposed for watermark adaptation: adapting the flow timing, and adapting the packet sizes. Experiments demonstrate that an adaptive watermark can survive  timing jitter two to three times more compared to similar non-adaptive watermarks using the same volume of traffic. 

Jin et al. develop a new metric to measure the effectiveness of anonymous networks \cite{conf/dsn/JinW09}. They use this measure to evaluate the effect of timing attacks on TOR anonymous networks. They find out that circuit rotation in TOR could significantly increase the its resistance to timing attack at the cost of more timing perturbations for the benign users. 


Ling et~al. in \cite{conf/ccs/LingLYFXJ09} propose a new attack the TOR network anonymity. The attack works by having an attacker   changing the cell counter of the target traffic marginally such that a secret data is inserted into the variations of the cell counters at a malicious exit node. An accomplice at  the entry node is then able to link senders/receivers by finding the inserted secret data from the cell counter information.  

The Quality of Service (QoS) of TOR anonymous system is analyzed in \cite{DBLP:conf/ipps/PriesYGF08}. The paper discovers several TCP performance degradation issues with TOR, by modeling the TOR TCP throughput and conducting real-world experiments.  \cite{journals/tpds/FuYJGG09} performs a similar approach to  analyze TCP performance issues of flow-based mix networks.  The paper finds that a mix's batching and reordering schemes can drastically reduce TCP throughput because of out-of-order packet delivery. The paper also proposes  new approaches to improve the TCP performance in such mix networks. 

Liu et al. in \cite{conf/ispec/LiuJL10} study existing IPD-based flow watermarks (this does not mention the  RAINBOW paper, though being very recent). The papers proposed to use weak signal detection model and cluster technology in order to avoid the need for precision time synchronization or packet number, that are an issue with previous schemes (again not mentioning RAINBOW). 

A novel flow-multiplication attack on TOR  is presented in \cite{DBLP:conf/cscwd/WangLYL09}, that is based on a fundamental vulnerability of anonymous web browsing, and performs man-in-the-middle attack on the HTTP traffic. The attack works by having a malicious TOR exit node  returning a anonymous webpage request by a rogue page containing a specific number of image tags. This makes the victim's browsing client to initiate deterministic number of web connections in order to fetch the images. An accomplice entry node can then link client and web server by finding such communication pattern. Even with all the active content systems being blocked by the client's browser the flow-multiplication attack can be effective by keeping the rogue connection running for longer time. 

Feigenbaum et~al. in \cite{DBLP:conf/pet/FeigenbaumJS10} consider the problem of active timing analysis against anonymous networks. Padding mechanisms which are used as countermeasures against timing attacks are foiled by an active adversary that insert delays and drop messages. The authors present a protocol that provides anonymity against active adversaries by using a black-box padding scheme for passive attackers. In other words, the scheme reduces the problem of anonymity against active attackers to padding against passive attackers. The protocol uses time-stamping to enforce timing patterns and redundancy to deal with both malicious and benign delays.   

Shah et~al. in \cite{Shah:woot09} propose a new covert channel, interference channel, that works by creating external interference on a shared communications network. The inference covert channel works by only jamming the candidate traffic for a short time and, unlike similar covert channels, does not need the covert sender to compromise an authorized sender or having the ability to send messages to the network. The scheme has particularly been suggested for watermarking of VoIP traffic, without any need to compromise routers or endpoints. 

Many existing timing analysis research are based on simulations or experiments on unrealistic local area networks. Daginawala et~al.\ develop SubRosa \cite{DBLP:conf/pet/DaginawalaW08}, an experimental platform for studying timing analysis attacks and defenses in low-latency anonymous networks. Based on the new experimental results, the paper also introduces spike analysis, a new timing analysis technique.  

Omar et~al.\ propose an intelligent host-based approach for the detection of stepping stones \cite{conf/wcecs_2009_II/153}. The scheme is based on Self-Organization Mapping (SOM), which provides unsupervised learning capability, yet is less complex compared to similar Artificial Intelligent approaches. Experimental results show that the scheme is able to detect stepping stones by only looking into the number of involved connection chain. Similarly, SOM is also used to design an intelligent network-based detection approach for stepping stones \cite{omar:WAS09}.  

Omar et~al.\ in \cite{omar:IJCSNS08} show through experiments by NS-2 that dropped packets influence the detection performance of stepping stone detectors, while many [of the pioneer] stepping stone detectors ignore the influence of such dropped packets in their algorithm design. 

Slotted packet counting attack is a passive correlation-based attack against anonymity protocols \cite{Fusenig09}. Due to the strong assumptions on the network setup, common packet counting attacks can easily lead to wrong conclusions. This is overcome in the slotted packet counting attack by accounting for the traffic load variation over the time. The attack is applicable to many anonymity protocols. 

Covert timing channels can  be reliably detected using entropy-based tests by measuring the anomalies in the shape and regularity of the flow timing. Walls et~al./ show that these detections can be foiled by a covert channel that intelligently manipulated the detection metrics \cite{Walls:tech09}. In particular, the paper introduces a  new covert timing channel, Liquid,  that smooths the distortions detected by the entropy-based tests using a portion of the inter-packet delays in a compromised stream. Experimental results confirms the undetectability of such timing covert channel while maintaining a reasonable throughput. 

Yi et~al.\ in \cite{DBLP:conf/uic/YiPWHH08} propose a watermark-based IP traceback scheme. A honeypot inserts digital watermarks into the candidate flow in order to make it possible to trace it back to the source of the connection.  

\cite{DBLP:journals/tpds/ZhuFGBZ10} considers correlation-based traffic analysis attacks on anonymity networks. Based on extensive experiments on time-domain and frequency-domain correlation methods the paper concludes that all but few batching strategies fail against flow-correlation attacks. Based on the empirical results, the authors give some advise on designing Mix networks  in order to counter flow-based correlation attacks.  


Pyun et~al.\ in \cite{DBLP:conf/broadnets/PyunR07} develop a method for optimizing the number and placement of  monitoring points for identifying the anonymised sources of attacks with minimum ambiguity. Different types of \textit{Graph separators}, i.e., vertex and edge separators,  are used to partition a network in order to put the monitors; the paper tries to optimize the number of such graph separators.  Experimental results show that with only $5\%$ of the ASes being monitored the source of an attack can  be identified with little ambiguity. ((perhaps this is useful for our covert communication research to allocate the place of covert proxies))    

\cite{Shullich-SS-Survey} is a survey on stepping stone detection which includes passive detection schemes, and early watermarking approaches. The report concludes with suggestions for the future research. 








